Understand the Dynamic World: An End-to-End Knowledge Informed Framework for Open Domain Entity State Tracking

Open domain entity state tracking aims to predict reasonable state changes of entities (i.e., [attribute] of [entity] was [before_state] and [after_state] afterwards) given the action descriptions. It's important to many reasoning tasks to support human everyday activities. However, it's challenging as the model needs to predict an arbitrary number of entity state changes caused by the action while most of the entities are implicitly relevant to the actions and their attributes as well as states are from open vocabularies. To tackle these challenges, we propose a novel end-to-end Knowledge Informed framework for open domain Entity State Tracking, namely KIEST, which explicitly retrieves the relevant entities and attributes from external knowledge graph (i.e., ConceptNet) and incorporates them to autoregressively generate all the entity state changes with a novel dynamic knowledge grained encoder-decoder framework. To enforce the logical coherence among the predicted entities, attributes, and states, we design a new constraint decoding strategy and employ a coherence reward to improve the decoding process. Experimental results show that our proposed KIEST framework significantly outperforms the strong baselines on the public benchmark dataset OpenPI.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> experiment_back0.tex <==


\section{Experiments}

\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 model&max-Length& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
		Paper gpt2 base&none & & & 3.6& & &13.4 & &&28.2\\
		GitHub-gpt2-base&400&8.82 & 7.00&4.13 &22.85 &19.08 & 16.38& 39.54&35.18 &32.66\\
        my-gpt2-base&400&8.85& 6.76&3.87 &22.77 &18.64 & 15.97& 39.75&34.51 &32.29\\
       
          % t5-large-baseline&400& 13.16   &7.46    & 5.06   & 32.02  &  22.42& 21.09 & 48.49 & 38.22 & 37.44\\
		\hline
        t5-large-baseline&400& 15.22  & 7.46  &  5.64 & 31.30 &20.33 & 19.29& 47.83&35.97 &35.52\\
        --decoder-entity-attr-no-pading&400&\textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
        % method1-add-attr&400& 16.85   &7.57   &6.30    &34.49   &22.06  & 21.53 &50.4 &36.88 & 36.99\\
        % method2-attr&400& 25.11   &6.15  &5.53    &39.54   &18.60 & 18.13 &54.37 &32.57 & 32.74\\
        \hline
        score$>$0.5&&    &   &    &   &  &  & & & \\
        --decoder-entity-attr-no-pading&400&\textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
        graph-rgcn-entity&400&    &   &    &   &  &  & & & \\
        graph-rgcn-attr&400& 25.11   &6.15   &5.53    &39.54   &18.60  & 18.18 &54.37 &32.57 & 32.74\\
        \hline
         graph-rgcn-attr-add&400& \textbf{16.85}   &\textbf{7.57 }  &\textbf{6.30 }   &\textbf{34.49}   &\textbf{22.06}  & \textbf{21.53 }&\textbf{50.40} &\textbf{36.88} & \textbf{36.99}\\
        --decoder-just-attr-4-tuple&400& \textbf{16.86}   &\textbf{7.58}   &\textbf{6.19}    &\textbf{34.57}   &\textbf{22.02} & \textbf{21.43} &\textbf{50.26} &\textbf{36.71} & \textbf{36.73}\\
         --decoder-just-entity-4-tuple&400& 15.58   &6.86   &5.15    & 31.54 &20.04 &18.90  &47.47 &34.98 &34.34 \\
         \hline
         --decoder-entity-attr-pading-0-postion&400& 24.28   &6.91   &5.51    & 38.49 &19.23 &18.20  &51.98 & 32.45&31.65 \\
          --decoder-entity-pading-0-postion&400&   &  &   &  & &  & & & \\
          --decoder-attr-pading-0-postion&400&    &  &    &  & &  & & & \\
          \hline
          --entity-attr-nopading-0-inside-atttention&400& 3.39   &3.75   &0.18    & 14.90 &14.83 &10.59  &31.54 & 31.39&27.13 \\
        \hline
        --decoder-entity-attr-no-pading&400&\textbf{ 20.04} &\textbf{ 7.26} & \textbf{6.64}  &\textbf{37.54}  &\textbf{21.47} &\textbf{21.68}  &\textbf{53.09} &\textbf{36.15} &\textbf{36.96} \\
        --decoder-entity-attr-no-pading&400&\textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
        --decoder-attr-no-pading&400&  &  &   &  & &  & & & \\
        --decoder-entity-no-pading&400& &  &   &  & &  & & & \\
        \hline
         --decoder-entity+attr-weighted-byits&400&  28.38&  6.77& 6.35  & 43.07 &19.29 &19.24  &56.57 &32.25 &32.63 \\
         \hline
        --decoder-just-attr&400& 27.46   &6.95   &6.78    &42.94   &19.67 & 20.06 &56.79 &32.64 & 33.58\\
 \hline
         
            transformer-attr&400& 19.38   &8.28   &7.04    &34.80   &21.74  & 20.76 &50.33 &36.74 & 36.15\\
         
 train-add-test-step&400& 26.50  &7.12   &6.95    &41.12   &19.62  & 19.80 &55.15 &32.76 & 33.43\\
         
         graph-rgcn-attr-two-decoder&400& 33.41   &6.70   &6.15     &46.70   &17.62  & 17.63 &59.22 &30. 36& 30.33\\
        graph-rgcn-all&400&    &   &    &   &  &  & & & \\
        \hline
        transformer-entity&400&    &   &    &   &  &  & & & \\
        transformer-attr&400&  49.89  & 5.29  &5.01    &58.29   &  12.37&  12.32&67.73 & 21.43& 21.59\\
        transformer-all&400&    &   &    &   &  &  & & & \\
    \hline
        rgcn-trans-entity&400&    &   &    &   &  &  & & & \\
        rgcn-trans-attr&400&    &   &    &   &  &  & & & \\
        rgcn-trans-all&400&    &   &    &   &  &  & & & \\
        
       \hline
        score $>$ 0.3&&    &   &    &   &  &  & & & \\
        graph-rgcn-entity&400&    &   &    &   &  &  & & & \\
        graph-rgcn-attr&400&    &   &    &   &  &  & & & \\
        graph-rgcn-all&400&    &   &    &   &  &  & & & \\
        n-graph-just-tra-fomer-all&400&    &   &    &   &  &  & & & \\
          \hline
            add constraint in output&&    &   &    &   &  &  & & & \\
        \hline
	\end{tabular}
 }
	\caption{Model performance}
\label{con:model-performance}
\end{table*}


==> experiment_back_2022_12_23.tex <==


\section{Experiments}
\subsection{Dataset}
We evaluate our model on an open domain state changes dataset OpenPI \cite{tandon2020dataset}, which is constructed  by crowdsourcing.  It has a different version for tracking state changes, with images and without images, in our work we only choose the version without images.
%%%%%%
There are two key points in the OpenPI dataset: 1) the surface names of \textit{Attribute, Entity, Beforestate} and \textit{Afterstate} are not always in the $q$, especially for the  \textit{ Beforestate, Afterstate}. such as question \textit{q}: \textit{Be in a fighting position with this person. Now, what happens?}, the 
 ground truth \textit{Entity}, such as "body" and "knee" are not in this question, the 
 ground truth \textit{state}, such as "down" and "up" is also not in this question. 2) In the testing dataset, not  all tuples (\textit{Attribute, Entity, Beforestate} and \textit{Afterstate}) are in the training set, and not all single elements (such as \textit{Attribute}) are in the training set. By statistics, in the tuples of testing data, there are 0.425 entities,  0.63 attributes, 0.49 before states, and 0.42 after states in the training data.
 The OpenPI dataset comprises 3216 sentences in the training set, 560 sentences in the testing data, and 274 sentences in the dev data.
\subsection{ Baselines and Evaluation matrixs}
 

 There is little work on this topic, so we validate our model by comparing [model name]'s performance with the recent work, and several commonly used models in the generation task, these models have achieved state-of-the-art performance. \textbf{OpenPI} \cite{tandon2020dataset} proposes to use GPT2-base model to generate the tuples directly. \textbf{T5-large (Fine-tune)} is fine-tuned on Common Crawl.
 \textbf{GPT2-large (Fine-tune)} is fine-tuned on event dataset.

Same as \cite{tandon2020dataset}, we use three commonly used overlap functions  Exact, BLEU, and ROUGE. The micro-averaged prediction, recall, F1 scores will be reported under each overlap function.

\subsection{Implementation details}
On NELL-ZS (or Wiki-ZS), each word in the surface name of  relation is set to $13$-gram (or $15$-gram) and the number of nodes in the n-gram graph is set to $90$ (or $70$). Each node in the n-gram graph is randomly initialized with a 200-dim embedding. The GramTransformer contains one multi-head attention block with three attention heads and a 200-dim feed-forward layer. The dropout rate in the multi-head attention and feed-forward layer is set to $0.5$.
Entities are also randomly initialized with 200-dim embeddings. During training, we use Adam sss as the optimizer and a Cross-entropy is used as the loss function with a learning rate of $0.0005$. We use label smoothing to prevent the model from becoming over-confident. All embeddings are fine-tuned during training.

\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 model&max-Length& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
		% OpenPI&none & & & 3.6& & &13.4 & &&28.2\\
		OpenPI\cite{tandon2020dataset}&400&8.82 & 7.00&4.13 &22.85 &19.08 & 16.38& 39.54&35.18 &32.66\\
  GPT2-large(Finetune)&400& 9.07 & 3.27 &3.33  &23.92   & 16.37 &  16.39 & 40.87 &32.06  &32.63 \\
        % OpenPI-gpt2-base&400&8.85& 6.76&3.87 &22.77 &18.64 & 15.97& 39.75&34.51 &32.29\\
          T5-large(Finetune)&400& \textbf{15.22 } & \textbf{7.46}  &  \textbf{5.64} & \textbf{31.30} &\textbf{20.33} & \textbf{19.29}& \textbf{47.83}&\textbf{35.97} &\textbf{35.52}\\
          % \hline
       T5-large-attr-ent-cat&400& 16.82 & 7.77  &  6.36 & 34.35 &20.31& 20.03&50.23 &35.00 &35.55\\
       \hline
          % t5-large-baseline-&400& 13.16   &7.46    & 5.06   & 32.02  &  22.42& 21.09 & 48.49 & 38.22 & 37.44\\
		
       
        % method1-add-attr&400& 16.85   &7.57   &6.30    &34.49   &22.06  & 21.53 &50.4 &36.88 & 36.99\\
        % method2-attr&400& 25.11   &6.15  &5.53    &39.54   &18.60 & 18.13 &54.37 &32.57 & 32.74\\
        \hline
         train(q,a,e)-pre(q,a,e)&400&   19.77  & 7.67 & 6.92  &37.66  &22.05 &22.17 &53.12 &36.63 &37.37 \\
        +constraint&400& \textbf{21.52}& 7.72   &  7.17&\textbf{ 39.73  }  &  22.53 & 22.92 &\textbf{54.77} & 37.10& 38.02\\
         +constraint\#reward&400& 20.91& \textbf{9.54}  & \textbf{ 7.84 } & 38.14    & \textbf{ 26.29}  &\textbf{ 24.24}  &53.43  & \textbf{40.77}& \textbf{39.40}\\
           \hline

	\end{tabular}
 }
	\caption{Model performance, OpenPI uses the gpt2-base model}
\label{con:model-performance}
\end{table*}



\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 model&max-Length& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
	
		% OpenPI\cite{tandon2020dataset}&400&8.82 & 7.00&4.13 &22.85 &19.08 & 16.38& 39.54&35.18 &32.66\\
  % GPT2-large(Finetune)&400& 9.07 & 3.27 &3.33  &23.92   & 16.37 &  16.39 & 40.87 &32.06  &32.63 \\
  %       % OpenPI-gpt2-base&400&8.85& 6.76&3.87 &22.77 &18.64 & 15.97& 39.75&34.51 &32.29\\
  %         T5-large(Finetune)&400& \textbf{15.22 } & \textbf{7.46}  &  \textbf{5.64} & \textbf{31.30} &\textbf{20.33} & \textbf{19.29}& \textbf{47.83}&\textbf{35.97} &\textbf{35.52}\\
  %         \hline
  %      T5-large-attr-ent-cat&400& 16.82 & 7.77  &  6.36 & 34.35 &20.31& 20.03&50.23 &35.00 &35.55\\
  %      \hline
          % t5-large-baseline-&400& 13.16   &7.46    & 5.06   & 32.02  &  22.42& 21.09 & 48.49 & 38.22 & 37.44\\
		
       
        % method1-add-attr&400& 16.85   &7.57   &6.30    &34.49   &22.06  & 21.53 &50.4 &36.88 & 36.99\\
        % method2-attr&400& 25.11   &6.15  &5.53    &39.54   &18.60 & 18.13 &54.37 &32.57 & 32.74\\
        \hline
        score$>$0.5&&    &   &    &   &  &  & & & \\
         train(q,a,e)-pre(q,a,e)&400& \textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
            train(q,e)-pre(q,e)&400& 17.49   & 7.86  &6.19    &34.95   &21.94  &21.00  &50.66 & 36.58& 36.41\\
        train(q,a)-pre(q,a)&400& 37.18  & 6.28  &5.22    &  50.02 &16.60  & 16.12 &62.23 &27.99 &28.05 \\

         

           train(q,a,e)-pre(q,a,e)-transformer&400&  22.86&  6.84 &    5.49&  39.62 & 19.64 & 19.27 & 54.37& 33.30&33.61 \\
           \hline
            score$>$0.3&&    &   &    &   &  &  & & & \\
               train(q,a,e)-pre(q,a,e)&400& 19.11 &  7.31     &5.98   & 35.91 & 20.85 &20.33 &51.68 &35.59 &35.69\\
            train(q,e)-pre(q,e)&400&  15.44 &  7.59& 6.01   &  32.84 & 21.91 & 21.05 &48.97 & 37.22&36.92 \\
          train(q,a)-pre(q,a)&400&  34.52 &  6.18 & 6.10   &  47.02 & 17.17 & 17.31 & 60.32& 29.92& 30.38\\

           train(q,a,e)-pre(q,a,e)-transformer&400& 16.96 & 7.61  &  5.72  &  33.79 & 21.18 & 20.08 & 49.63& 36.47& 35.77\\
           \hline
    train(q,a,e)-pre(q,a,e)-no-filter&400& 12.90 & 7.67  &  5.58  & 30.36  &22.78  & 21.08 & 47.24&38.48 &37.42 \\
           \hline
	\end{tabular}
 }
	\caption{Model performance, OpenPI uses the gpt2-base model}
\label{con:model-performance}
\end{table*}





% this filter is not good, why using this method is invalid (we cannot see this filter is invalid because we used it before)?


% 1-no-train:so the next just using the sentence embedding to calculate the embedding.

% 2-tf-idf

% 3-different sentences set the  different threshold

% to check how to filter the candidate

% what is the difference between the first filter, to score the entity in the retrieved entity,

% but now the candidate set is t5 filted



\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 score&Constraint& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
  OpenPI\cite{tandon2020dataset}&400&8.82 & 7.00&4.13 &22.85 &19.08 & 16.38& 39.54&35.18 &32.66\\
  GPT2-large(Finetune)&400& 9.07 & 3.27 &3.33  &23.92   & 16.37 &  16.39 & 40.87 &32.06  &32.63 \\
        % OpenPI-gpt2-base&400&8.85& 6.76&3.87 &22.77 &18.64 & 15.97& 39.75&34.51 &32.29\\
          T5-large(Finetune)&400& 15.22  & 7.46  &  5.64 & 31.30 &20.33 & 19.29&47.83&35.97 &35.52\\
-&T5 Dict& \textbf{ 19.77} & \textbf{7.67}& \textbf{6.92} &\textbf{37.66} &\textbf{22.05} &\textbf{22.17} & \textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
\hline
  -&T& 50.54  & 4.66  & 4.27   & 57.77  & 9.72 &  9.89&65.40 & 17.26& 17.62\\
    -&GE&  62.21 &  5.31 &  5.07  &  69.37 & 10.64 & 10.92 & 75.74& 17.34&17.69 \\
 -&T+GE&  40.16    & 5.72  & 5.55     &51.55   &14.15    & 14.72& 61.50 &24.23 &24.97 \\
\hline

     0.2&FT5&\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\

     
      0.2&FT5+GE&\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\
      
        
 0.2&FT5+T&\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\
     0.2& FT5+GE+T  &\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\
% 0.2& filter-char   &\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02} \\
% 0.2& FT5+GE+T-   &\textbf{ 16.26}&\textbf{ 7.69 }  & \textbf{ 6.90 } & \textbf{34.14  }  & \textbf{ 22.51}  &\textbf{ 22.46}  &\textbf{50.44}  & \textbf{37.88}&\textbf{ 38.45 }\\

% 0.2& New  &\textbf{ 20.37}&\textbf{ 7.69 }  & \textbf{ 7.44 } & \textbf{37.69  }  & \textbf{ 22.10}  &\textbf{ 22.55}  &\textbf{53.28}  & \textbf{36.90}&\textbf{ 37.92 }\\
% 0.2& FT5+T   &\textbf{ 20.73}&\textbf{ 7.69 }  & \textbf{ 7.80 } & \textbf{38.04  }  & \textbf{ 22.10}  &\textbf{ 22.91}  &\textbf{53.64}  & \textbf{36.90}&\textbf{ 38.28 }\\
% 0.2& FT5+GE+T  &\textbf{ 20.73}&\textbf{ 7.69 }  & \textbf{ 7.80 } & \textbf{38.04  }  & \textbf{ 22.10}  &\textbf{ 22.91}  &\textbf{53.64}  & \textbf{36.90}&\textbf{ 38.28 }\\
% 0.2& FT5+GE+T-remove-char  &\textbf{ 21.29}&\textbf{ 8.50}  & \textbf{ 7.97 } & \textbf{41.08  }  & \textbf{ 23.89}  &\textbf{ 24.60}  &\textbf{56.12}  & \textbf{38.30}&\textbf{ 39.65}\\
\hline

     0.4&FT5&\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\
      0.4&FT5+GE&\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\
 0.4&FT5+T&\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\
     0.4& FT5+GE+T  &\textbf{ 21.52}& \textbf{7.72 }  & \textbf{ 7.17 } & \textbf{39.73}    & \textbf{ 22.53}  &\textbf{ 22.92}  &\textbf{54.77}  & \textbf{37.10}& \textbf{38.02}\\

\hline
     0.6&FT5&20.30    & 7.40  &   6.92  &  37.74 &21.63    & 21.91  & 53.38  & 36.31 & 37.28 \\  
      0.6&FT5+GE& 20.44   & 7.62  & 7.25    &  38.40 &22.12    & 22.64  & 53.77  &36.89  & 37.96 \\
 0.6&FT5+T& 20.44   & 7.62  & 7.25    &  38.40 &22.12    & 22.64  & 53.77  &36.89  & 37.96 \\
     0.6& FT5+GE+T  & 20.44   & 7.62  & 7.25    &  38.40 &22.12    & 22.64  & 53.77  &36.89  & 37.96 \\
         \hline
    0.8&FT5&  36.52   &6.83   & 5.99   & 50.43   &   17.93  & 17.81   & 62.80   & 29.56 &29.99   \\  
      0.8&FT5+GE& 28.71    & 6.82  &6.19    & 43.89   &  18.91   &  19.00  & 57.92   & 32.04 & 32.67  \\
 0.8&FT5+T& 25.19    & 7.23  &   6.49 & 40.81  & 19.45 &19.62     & 55.21   &  32.98  & 33.74   \\
     0.8& FT5+GE+T& 24.88    & 7.32  &  6.60  & 41.02   & 20.14    &  20.34  &  55.74  &33.96  & 34.75  \\
         \hline
	\end{tabular}
 }
	\caption{The model performance under different relevant scores. In the constraint, T refers to the $AKS$ and $EKS$ is the entity set and attribute set in the train data, GE  refers to the $AKS$ and $EKS$ is the retrieved  entity and attribute, FT5 refers to the $AKS$ and $EKS$  is the filtered t5 token set. }
\label{con:model-performance}
\end{table*}


\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 score&Constraint& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
0&T5 Dict&  19.77 & 7.67& 6.92 &37.66 &22.05 &22.17 &53.12 &36.63 &37.37 \\
\hline
     0.2&FT5& 36.20  & 6.70  & 5.71   & 47.90   & 16.78  & 16.04 &60.89 &28.83  &  28.61 \\
      0.2&FT5+GE& 36.29  &6.32   & 5.44   &   49.06 & 17.11  & 16.56 & 61.53& 28.79 &  28.72 \\
 0.2&FT5+T& 36.28  & 6.20  &  5.43  & 49.54   &16.88   & 16.74 & 62.00& 28.82 & 29.07  \\
     0.2&FT5+GE+T&  38.06 &  6.03 & 5.24   &  50.31  & 16.07  & 15.72 &62.60 & 27.65 & 27.82  \\
\hline
     0.4&FT5& 36.20  &  6.70 &   5.71 &47.90    &  16.78 & 16.04 &60.89 & 28.83 & 28.61  \\
      0.4&FT5+GE& 36.29  & 6.32  &5.44    &  49.06  & 17.11  & 16.56 & 61.53& 28.79 &28.72   \\
 0.4&FT5+T& 36.28  & 6.20  &   5.43 &   49.54 & 16.88  & 16.74 & 62.00& 28.82 &  29.07 \\
     0.4& FT5+GE+T & 38.06  & 6.03  &5.24    &  50.31  &  16.07 & 15.72 &62.60 &27.65  & 27.82  \\
\hline
     0.6&FT5&  36.20 &6.70   &  5.71  &  47.90  & 16.78  & 16.04 & 60.89& 28.83 & 28.61  \\
      0.6&FT5+GE&36.29   & 6.32  & 5.44   &  49.06  & 17.11  & 16.56 & 61.53& 28.79 & 28.72  \\
 0.6&FT5+T& 36.28  &6.20   &  5.43  &49.54    &16.88   &16.74  &62.00 & 28.82 &29.07   \\
     0.6& FT5+GE+T  & 38.06  & 6.03  & 5.24   & 50.31   & 16.07  & 15.72 &62.60 &27.65  & 27.82  \\
         \hline
  0.8&FT5& 35.42  & 6.03  &  4.63  & 47.18   &   15.67& 14.67 &59.95 &27.67  &  27.17 \\
      0.8&FT5+GE& 35.67  &6.57   & 5.61   & 48.94   & 17.20  &16.82  &61.88 & 29.29 & 29.50  \\
 0.8&FT5+T&38.70   &  6.16 &   5.43 &  50.79  & 15.94  & 15.76 &63.27 &27.43  &27.74   \\
     0.8& FT5+GE+T & 34.89  & 6.31  & 5.53   &  48.20  & 17.40  & 17.09 &60.95 & 29.45 &29.63   \\
         \hline
       
	\end{tabular}
 }
	\caption{Tree structure}
\label{con:model-performance}
\end{table*}

\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 Constraint& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
T5 Dict&  19.77 & 7.67& 6.92 &37.66 &22.05 &22.17 &53.12 &36.63 &37.37 \\
\hline
 T& 38.74  &  5.86 & 5.67   & 50.38  &  14.82&  15.37&62.60 &26.15 & 27.34\\
GE&38.67   & 5.98  &5.56    & 51.34  &15.17  &15.77  & 63.62& 26.51&27.77 \\
T5& 36.20  &6.70   &  5.71  & 47.90  &16.78  &16.04  &60.89 &28.83 & 28.61\\
 T5+GE&  36.29 & 6.32  & 5.44   & 49.06  &17.11  & 16.56 & 61.53&28.79 & 28.72\\
T5+T&  36.28 & 6.20  & 5.43   &49.54   &16.88  &16.74  &62.00 &28.82 & 29.07\\
 T5+GE+T   &  38.06 &  6.03 &5.24    & 50.31  &16.07  & 15.72 &62.60 &27.65 & 27.82\\
         \hline
	\end{tabular}
 }
	\caption{Tree structure, T5 dictionary}
\label{con:model-performance}
\end{table*}


\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 score&Constraint& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
0&T5 Dict&  19.77 & 7.67& 6.92 &37.66 &22.05 &22.17 &53.12 &36.63 &37.37 \\
\hline


    prompt2-question&400&  6.06 &  7.95 &   4.52 & 24.70  & 24.74 &21.41  & 42.76& 41.93& 39.12\\
    no prompt1-[SN]--[END]&400&17.78   & 7.24  &6.45    & 35.50  & 21.02 &  21.27& 51.72& 35.80&36.81 \\
    prompt1-[SN]--[END]&400&  8.24 & 7.63  & 4.95   &  27.14 & 23.40 &21.37  & 44.86&39.66 &38.48 \\
     no-prompt-no-kg-<attr>&400&   &   &    &   &  &  & & & \\
         \hline
	\end{tabular}
 }
	\caption{Prompt is good or not Model performance, prompt1: " attribute of entity was old state before and new state afterwards", prompt2:" <attr> [attribute] </attr> of <entity> [entity] </entity> was [before state] before and [after state] afterwards",------(1): just reserve the word which has english letter (▁préféré	22157) will be removed,  (2) reserve the English word, tool is not good}
\label{con:model-performance}
\end{table*}



% \begin{table}[h]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% 	\begin{tabular} {lccc}
% 		\hline
		
% 		\hline
% 		& train/ml&test/ml&dev/ml\\ 
% 		\hline	
%             % entity type&  & & \\ 
%             \multicolumn{4}{c}{entity type}\\
%             \hline	
%             no-filter& 0.60/9k &0.70/28k & 0.65/28k\\ 
%             filter-0.3& 0.60/3k &0.69/17.5k  & 0.65/13k\\ 
%            filter-0.3-rs& 0.60/2984 & 0.68/12.5k & 0.63/9023\\
%            filter-0.5& 0.54/1k &0.62/9k & 0.58/6k\\ 
%            filter-0.5-rs& 0.52/1k & 0.60/6k& 0.56/2975\\
% 		 % attr& 0.90/0.82/0.79 & 0.90/0.81/- &0.91/0.81/- \\ 
% 		\hline
%         \multicolumn{4}{c}{attribute type}\\
% 		 % attribute type&  & & \\ 
%             \hline	
%             no-filter& 0.82/9k& 0.90/28k &0.91/28k\\ 
%             filter-0.3& 0.80/350 &0.83/800  & 0.88/800\\ 
%            filter-0.3-rs& 0.71/350 & 0.79/566 & 0.83/538\\
%            filter-0.5& 0.76/140&0.80/400 & 0.85/500\\ 
%            filter-0.5-rs& 0.67/123 & 0.71/215 & 0.72/163\\    
% 		\hline
% 	\end{tabular}
% 	\caption{The recall value about retrieved entities  with 2 hops in ConceptNet. $rs$ refers to removing the single node. $ml$ refers to the max length of retrieved entities. 
%   In filter-$n$, $n$ refers to the similarity between the question and entity.}\label{ref:filter-score-hop2}
% \end{table}
% \begin{table}[h]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% 	\begin{tabular} {lccc}
% 		\hline
		
% 		\hline
% 		& train/ml&test/ml&dev/ml\\ 
% 		\hline	
%             entity type&  & & \\ 
%             \hline	
%             no-filter&  0.55/2938  &0.56/2849  & 0.53/2601  \\ 
%             filter-0.3& 0.48/1009  &0.54/1625   & 0.51/ 1202 \\  
%            filter-0.3-rs&  0.48/1009  &0.54/1625   & 0.51/ 1202  \\ 
%            filter-0.5&  0.44/428  &0.49/ 914  & 0.47/636  \\ 
%            filter-0.5-rs&  0.44/428  &0.49/914   & 0.47/636   \\ 
% 		 % attr& 0.90/0.82/0.79 & 0.90/0.81/- &0.91/0.81/- \\ 
% 		\hline
% 		 attribute type&  & & \\ 
%             \hline	
%             no-filter&  0.32/2938  &0.34/2849   & 0.32/2601  \\ 
%             filter-0.3&  0.28/119  &0.29/ 125  & 0.30/128  \\ 
%            filter-0.3-rs&  0.28/119  &0.29/ 125  & 0.30/128   \\ 
%            filter-0.5&  0.27/48  &0.28/75   & 0.29/ 54 \\  
%            filter-0.5-rs&  0.27/48  &0.28 /75   &0.29/ 54 \\   
% 		\hline
% 	\end{tabular}
% 	\caption{The recall value about retrieved entities  with 1 hops in ConceptNet. $rs$ refers to removing the single node. $ml$ refers to the max length of retrieved entities. 
%   In filter-$n$, $n$ refers to the similarity between the question and entity.}\label{ref:filter-score}
% \end{table}


 % By statistics, in the testing data of OpenPI, we found there are 0.70 ground entities and 0.90 ground attributes in the retrieved entities of Hop2, while there are 0.60 ground entities and 0.82 ground attributes in the retrieved entities of Hop2.
 % More  intuitively, the knowledge stored in KG can help generation model obtain  the implicitly mentioned entities or attributes. For example,  as shown in Figure \ref{fig:whole framework},  the target entities \textit{body, muscle, hand} with the target attributes \textit{position, energy, placement} will be obtained  by the enumeration method within Hop2. So, we assume retrieved knowledge can help improve the model performance.

 
% Specifically, to train the entity filter $f_{e}$, for each action description $x_q$=\{$w_0$, $w_1$, $w_2$, $\cdots$, $w_m$\}, where $w_m$ is the $m$-th token of $x_q$, we first obtain a set of positive entities\footnote{The positive answer entities of  question can be found from the answers provided in OpenPI, in its answer template: \textit{A of E was S1 before and S2 afterwards},  \textit{ A} is the attribute, \textit{E} is the entity.} 
% $t^p$=\{$e_0$, $e_1$, $e_2$, $\cdots$, $e_n$\}, where each $e_i$ is extracted from a particular state change annotation for $x_q$. We take all the other entities that are included in $E_{x_q}$ but not included in $t^p$ as negative entities: $t^n=E_{x_q}-t^p$.\lifu{clean and redesign these math symbols to make them self-explainable}. In order to train the entity filter, we take

==> experiments_back1.tex <==


\section{Experiments}

\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 model&max-Length& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
		Paper gpt2 base&none & & & 3.6& & &13.4 & &&28.2\\
		GitHub-gpt2-base&400&8.82 & 7.00&4.13 &22.85 &19.08 & 16.38& 39.54&35.18 &32.66\\
        my-gpt2-base&400&8.85& 6.76&3.87 &22.77 &18.64 & 15.97& 39.75&34.51 &32.29\\
          t5-large-baseline&400& \textbf{15.22 } & \textbf{7.46}  &  \textbf{5.64} & \textbf{31.30} &\textbf{20.33} & \textbf{19.29}& \textbf{47.83}&\textbf{35.97} &\textbf{35.52}\\
       
          % t5-large-baseline-&400& 13.16   &7.46    & 5.06   & 32.02  &  22.42& 21.09 & 48.49 & 38.22 & 37.44\\
		
       
        % method1-add-attr&400& 16.85   &7.57   &6.30    &34.49   &22.06  & 21.53 &50.4 &36.88 & 36.99\\
        % method2-attr&400& 25.11   &6.15  &5.53    &39.54   &18.60 & 18.13 &54.37 &32.57 & 32.74\\
        \hline
        score$>$0.5&&    &   &    &   &  &  & & & \\
         train(q,a,e)-pre(q,a,e)&400& \textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
            train(q,e)-pre(q,e)&400& 17.49   & 7.86  &6.19    &34.95   &21.94  &21.00  &50.66 & 36.58& 36.41\\
        train(q,a)-pre(q,a)&400& 37.18  & 6.28  &5.22    &  50.02 &16.60  & 16.12 &62.23 &27.99 &28.05 \\

          train(q,a,e)-pre(q,a,e)-no-filter&400&   &   &    &   &  &  & & & \\

           train(q,a,e)-pre(q,a,e)-transformer&400&   &   &    &   &  &  & & & \\
           \hline
            generation-constraint-no-end&&   &   &    &   &  &  & & & \\
             all-knowledge-constrant-e-ground&400& 19.62  & 8.11  &8.12    &  39.55 & 23.82 &25.01  &55.33 & 38.79&40.68 \\
          all-knowledge-constrant-e&400&   &   &    &   &  &  & & & \\
           all-knowledge-constrant-a&400&   &   &    &   &  &  & & & \\
            all-knowledge-constrant-all&400&   &   &    &   &  &  & & & \\
            \hline
            generation-constraint-end-token&&   &   &    &   &  &  & & & \\
          all-knowledge-constrant-e&400&   &   &    &   &  &  & & & \\
           all-knowledge-constrant-a&400&   &   &    &   &  &  & & & \\
            all-knowledge-constrant-all&400&   &   &    &   &  &  & & & \\
       \hline
	\end{tabular}
 }
	\caption{Model performance}
\label{con:model-performance}
\end{table*}


\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 Constraint&Recall& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
        score$>$0.5&&    &   &    &   &  &  & & & \\
        just-e&&    &   &    &   &  &  & & & \\
              generation-constraint-no-token&&   &   &    &   &  &  & & & \\
              t5-large-baseline&400& \textbf{15.22 } & \textbf{7.46}  &  \textbf{5.64} & \textbf{31.30} &\textbf{20.33} & \textbf{19.29}& \textbf{47.83}&\textbf{35.97} &\textbf{35.52}\\
              
         T5-dict&0.7084& \textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
      
        entity-ground&1&\textbf{ 19.62} & \textbf{8.11}  &\textbf{8.12 }   &  \textbf{39.55} & \textbf{23.82} &\textbf{25.01}  &\textbf{55.33} & \textbf{38.79}&\textbf{40.68} \\

        entity-groud_2&1&\textbf{ 21.29} & \textbf{8.50}  &\textbf{7.97 }   &  \textbf{41.08} & \textbf{23.89} &\textbf{24.60}  &\textbf{56.12} & \textbf{38.30}&\textbf{39.65} \\
        entity-attr-groud_2&1&\textbf{ 21.38} & \textbf{8.26}  &\textbf{7.88 }   &  \textbf{41.06} & \textbf{24.07} &\textbf{24.73}  &\textbf{56.12} & \textbf{38.75}&\textbf{39.97} \\
     
          fitled-entity&0.6026&19.51   &7.52   &6.22    & 36.06  &21.54  &20.81  &51.49 &36.03 & 35.90\\
           train entity set&0.650& 19.86  & 7.32  &6.69    &36.36   & 21.22 &21.19  &52.29 & 36.09& 36.74\\
            t5-dict+filted entity&0.7558&  19.40 &  7.52 & 6.36   & 36.26  &20.72  & 20.47 &52.00 &35.75 & 36.08\\
            t5-dict+train entity set&0.7798&20.59   &  7.46 &  6.17  & 36.94  &21.08  & 20.48 & 52.39&35.87 & 35.74\\
        filted entity+train entity set&0.7217& 19.38  & 7.68  & 6.82   & 35.85  & 21.51 &  21.24&51.67 &36.31 &36.73 \\
        filted entity+train entity set +t5 dict&0.80& 19.13  & 7.63  &6.84    &35.92   &21.29  & 21.26 & 51.62&36.24 &36.74 \\
        \hline
           entity+attr+ground&1&\textbf{ 21.41} & \textbf{8.34}  &\textbf{8.73 }   &  \textbf{41.38} & \textbf{23.69} &\textbf{25.40}  &\textbf{56.82} & \textbf{38.14}&\textbf{40.62} \\
           attr-ground&1&20.18& 7.74  & 6.82  & 37.42   &21.87   & 21.75 & 53.17 &36.95 & 37.40 \\
        attr-ground2&1&19.07  & 7.63 & 6.69  &36.53   & 21.58 & 21.58 &52.42 & 36.68 &37.26\\

           
           filted-attr&&   &   &    &   &  &  & & & \\
           train attr set&0.91089&  19.70 & 7.78  &  6.55  & 37.22  & 22.25 &21.67  & 52.84&37.05 &37.15 \\
           t5+filed attr& 0.9445& 20.11  & 7.59  &  6.99  & 36.55  &21.48  & 21.45 &52.58 &36.43 &37.06 \\
           t5+train attr&0.98883& 21.15  &7.44   & 7.05   & 37.93  & 21.59 &21.77  & 53.67&36.40 &37.23 \\
           filted attr+ train attr set&0.912&   20.48& 7.67  & 6.21   & 38.17  & 21.92 & 21.30 & 53.50&36.80 & 36.68\\
 t5-remove(--) and lower& &  20.21& 7.31  & 68.7   & 36.65  & 21.11 & 21.22 & 52.78&36.09 & 36.88\\


           
          %   \hline
          %   filted entity+train attr+t5 dict&&   &   &    &   &  &  & & & \\
          % all-knowledge-constrant-e&400&   &   &    &   &  &  & & & \\
          %  all-knowledge-constrant-a&400&   &   &    &   &  &  & & & \\
          %   all-knowledge-constrant-all&400&   &   &    &   &  &  & & & \\

            
       \hline
prompt2-question&400&  6.06 &  7.95 &   4.52 & 24.70  & 24.74 &21.41  & 42.76& 41.93& 39.12\\
no prompt1-[SN]--[END]&400&17.78   & 7.24  &6.45    & 35.50  & 21.02 &  21.27& 51.72& 35.80&36.81 \\
prompt1-[SN]--[END]&400&  8.24 & 7.63  & 4.95   &  27.14 & 23.40 &21.37  & 44.86&39.66 &38.48 \\
 no-prompt-no-kg-<attr>&400&   &   &    &   &  &  & & & \\

        \hline
        \textbf{New-Results} from token level&&   &   &    &   &  &  & & & \\
T5-dict&1& \textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
 filted-T5+G-entity+train-entity(1)&0.99910&\textbf{ 20.01}&\textbf{ 7.69 }  & \textbf{ 7.08 } &\textbf{ 37.33}    & \textbf{ 22.10}  &\textbf{ 22.19}  &\textbf{ 52.92}  & \textbf{ 36.90}&\textbf{ 37.56} \\

filted-T5+G-entity+train-entity(2)&0.9931&20.98&8.12   & 7.22  & 37.76   & 21.79  &  21.66&52.93  &36.22 & 36.64 \\

ground&1&19.50&7.83  & 6.82 & 39.19 & 23.09  &  23.25&55.15  &38.19& 39.10 \\


0.03&--&20.01&7.69   & 7.08  &37.33    & 22.10  &22.19  &52.92  & 36.90&37.56 \\
0.04&--&20.01&7.69   & 7.08  &37.33    & 22.10  &22.19  &52.92  & 36.90&37.56 \\
0.05&--&20.01&7.69   & 7.08  &37.33    & 22.10  &22.19  &52.92  & 36.90&37.56 \\
0.08&--&20.01&7.69   & 7.08  &37.33    & 22.10  &22.19  &52.92  & 36.90&37.56 \\
0.09&--&21.00&7.68   & 7.20  &38.20    & 21.62  &21.91  &53.55  & 36.17&37.11 \\
0.095&--&19.86&7.62   & 6.73  &37.30    & 22.18  &21.91  &52.78  & 36.80&37.20\\
filted-T5+--0.1&--&19.86&7.62   & 6.73  & 37.30   & 22.18  &  21.91&52.78  &36.80 & 37.20 \\
0.2&--& 21.48  & 7.45  &6.95    &38.79   & 21.73 & 21.90 &54.35 &36.28 & 37.16\\
0.3&--&  21.11 &  7.37 & 6.39   &38.06   &20.97  &20.86  &53.17 &35.11 &35.64 \\
0.4&--&  21.07 & 7.41  &6.60    &38.79   &21.57  &21.61  &54.02 &36.06 &36.71 \\
>0.5&--&20.70   &7.40   &6.60    & 37.95  &21.18  &21.22  &53.52 &35.69 &36.41 \\
         \hline
	\end{tabular}
 }
	\caption{Model performance, prompt1: " attribute of entity was old state before and new state afterwards", prompt2:" <attr> [attribute] </attr> of <entity> [entity] </entity> was [before state] before and [after state] afterwards",------(1): just reserve the word which has english letter (▁préféré	22157) will be removed,  (2) reserve the English word, tool is not good}
\label{con:model-performance}
\end{table*}



this filter is not good, why using this method is invalid (we cannot see this filter is invalid because we used it in the before)?


1-no-train:so the next just using the sentence embedding to calculate the embedding.

2-tf-idf

3-different sentences set the  different threshold

to check how to filter the candidate

what is the difference between the first filter, to score the entity in the retrieved entity,

but now the candidate set is t5 filted
\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 Constraint&Recall& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
         1-fitled entity--other p source t5 dict&&   &   &    &   &  &  & & & \\
T5-dict&1& \textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\



0.2& 0.99899   &\textbf{ 20.01}&\textbf{ 7.69 }  & \textbf{ 7.08 } &\textbf{ 37.33}    & \textbf{ 22.10}  &\textbf{ 22.19}  &\textbf{ 52.92}  & \textbf{ 36.90}&\textbf{ 37.56}  \\
0.3&0.99853& 20.94  &7.38   &6.81    &38.18   &21.40  &21.54  &53.54 &36.08 &36.79 \\
0.4&0.99207& 21.53  &7.59   &6.67    &38.23   &21.00  &21.02  &53.55 &35.49 &36.02 \\
0.5&0.98355& \textbf{21.28 } &\textbf{7.67}   &\textbf{7.43}    &\textbf{38.42 }  &21.78 &\textbf{22.28 } &\textbf{53.51} &36.27 &37.28 \\
0.52&& 21.19  &7.30   &6.36    &  38.42 & 21.15 & 21.02 &53.80 &35.63 &36.14 \\
  0.54&& 20.93  & 7.41  &  6.63  &  38.07 & 21.26 & 21.33 &53.31 &35.53 & 36.23\\
    0.55&& 20.25  & 7.26  &  6.55  &37.53   & 21.42 &  21.43& 52.88&35.95 &36.59 \\
      0.56&& 21.21  & 7.71  &    6.89& 37.76  & 21.40 &21.27  &52.96 &36.09 & 36.41\\
        0.57&&22.32   &7.88   & 7.24   &39.04   & 21.41 &21.62  &53.95 & 35.51& 36.26\\
0.6&0.9764& 22.91  &7.73   &6.79    &39.19   &20.89  &20.80 &54.38 &34.75 &35.39 \\

0.7&0.9700& 20.22  &7.82   &7.10    &37.15   &21.39  &21.55 &52.69 &35.96 &36.79 \\
\hline
  2-fitled attr--other p source t5 dict&&   &   &    &   &  &  & & & \\
  0.2& & \textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
  0.21&&20.17   & 7.62  & 6.62   & 38.12  &22.05  & 21.90 &53.58 &36.69 &37.15 \\
0.26-8&&19.46   & 7.29  & 6.51   & 37.30  &21.53  & 21.61 &52.91 &36.53 &37.12 \\
  0.3&&20.74   &7.65   &6.43    &38.11   &21.67  &21.23  &53.37 &36.35 &36.47 \\
  0.4&&20.54   &7.21   &6.27    &36.54   &20.25  &20.06  &51.78 &34.51 &34.90 \\
  0.5&&  18.13 & 7.17  &5.71    &34.02   &19.97  &19.27 &49.63 &34.86 & 34.71 \\
  0.6&& 20.02  & 6.44  &5.73    &36.06   &19.21  &19.21  &51.00 &33.59 &34.16 \\
  0.7&& 19.17  &6.65   &5.67    & 35.00  &19.60  &19.32  &50.43 &34.48 & 34.67\\
\hline
3-all&&   &   &    &   &  &  & & & \\
0.2&    &\textbf{ 20.01}&\textbf{ 7.69 }  & \textbf{ 7.08 } &\textbf{ 37.33}    & \textbf{ 22.10}  &\textbf{ 22.19}  &\textbf{ 52.92}  & \textbf{ 36.90}&\textbf{ 37.56}  \\
0.5&& 20.15  &6.89   &6.38    &35.99   &19.64  &19.86  &51.27 &33.96 &34.88 \\

         \hline
         4-all-other position word&&   &   &    &   &  &  & & & \\
all-4&& 19.10 &7.48  &6.61    &36.92   &21.70  &21.83  &52.81 &36.91 &37.55 \\
         \hline
	\end{tabular}
 }
	\caption{New--2022-11-9}
\label{con:model-performance}
\end{table*}


==> method_back_2023_1_3.tex <==

Our model generates the template answers via a  transformer-based encoder-decoder architecture, integrating the retrieved entities and attributes  through the cross-attention  as introduced \cite{vaswani2017attention}. Given the token  sequence 
question $x$=\{$w_0$, $w_1$, $w_2$, $\cdots$, $w_m$\} as input, KGCR-EST   generates the linearized answer token $y$=\{$o_0$, $o_1$, $o_2$, $\cdots$, $o_m$\}. To this end, in the first, our model calculates the hidden semantic representation $QK$=\{$h_0$, $h_1$, $h_2$, $\cdots$, $h_m$\} of the input question $q$ via the encoder block in the multi-layer transformer:
\begin{align}
QK=Encoder(w_0, w_1, w_2, \cdots, w_m)
\end{align}
where $QK \in \mathbb{R}^{m \times d}$, in each layer, $Encoder(.)$ is an encoder block  in transformer by utilizing the multi-head attention mechanism.

After inputing action descriptions, filtered entities, and filtered attributes are encoded, our proposed Multi-Knowledge Decoder (MKDecoder) predicted the output answers token-by-token with the three types of input knowledge. At the step $i$ of generation, the decoder predicts the $i$-th token $o_i$ in the linearized form, and the decoder state $h_i^d$ as:
\begin{align}
o_i,h_i^d=F([QK,EK,AK,(h_i^0,\cdots,h_{i-1}^d)],o_{i-1})
\end{align}
where $F(.)$ denotes the MKDecoder.
In the next section, we will describe MKDecoder in detail.

==> method_back_2023_1_6.tex <==
% \section{Methodology\lifu{either use Approach or the full name of KIEST}}

\section{Methodology}
% \lifu{when defining new names, use command, e.g., \textsc{Kiest} to highlight it}



% \subsection{Overview}
% \lifu{In the original setting of OpenPI, they have two types of input: Context, and Query. Did you also use the context?}
\paragraph{ Task Description}
Given a procedural paragraph with a sequence of action descriptions, we aim to predict all the state changes of entities related to each action. We follow~\cite{tandon2020dataset} and formulate the task of open domain entity state tracking as follows. The \textbf{Input} $x=(x_q,x_c)$ consists of a \textit{context} $x_c$
% \lifu{define a math symbol} 
that includes one or a few history action descriptions and a \textit{query} $x_q$ that is the concatenation of a description for the current action and a short question ``\textit{what happens?}'', and the \textbf{Output} is a set of entity state changes $\mathbf{s}=\{s_j\}$ while each $s_j$ follows a template: [\textit{attribute}] \textbf{of}  [\textit{entity}] \textbf{was}  [\textit{before\_state}] \textbf{before and}  [\textit{after\_state}] \textbf{afterwards}. 

%%%%%%%%%%%%%%%overview

\paragraph{Overview}
%%% motivation
Intuitively, when asked to write state changes with a given action description, humans will always call to mind the scenarios associated with the anchors in the description, then conceive logical entity, attribute, and states\footnote{Note: There is no open KG to describe the state changes for the entity, so in our work, we only explore the effectiveness of introducing the entity and attribute knowledge on our model}, in further, for the special element (e.g.entity, attribute) in the entity state changes, humans always automatically select the corresponding knowledge for these elements.
For example, when writing to an entity in the state change, humans will always  call to mind the relevant entity knowledge. Similarly, our framework retrieves entities and attributes related to the given description from external KG, then uses them as auxiliary information for the state change generation. 
% Our KIEST framework aims to dynamically incorporate the entity and attribute knowledge obtained from KG to guide the entity state tracking task.
%%%%%%%%%  which contains abundant knowledge
More specially,
Figure~\ref{fig:whole framework} illustrates the overall architecture of our framework, which accepts a token description, and the entities and attributes in its \textsl{entity-attribute knowledge graph (KG)}
% \lifu{names such as Description KG are very awkward. Readers won't get the meaning of such names and if so, they will give a very low score to the clarity. Just imagine yourself as a reader and what's your feeling when you see such names that you don't understand} 
as input. The entity-attribute KG is firstly created by the \textbf{Entity-Attribute Retrieval and Scorer} module, where the nodes in the graph can be further decomposed into  entity nodes and attribute nodes.
% \lifu{when describing the approach, especially the overview, always first talk about the motivation or goal, then describe what you do. Otherwise, readers won't understand why you do this}. 
Next, the token sequence is encoded by a multi-layer transformer-based encoder. The output of the encoder is further used as input for the \textbf{Dynamic knowledge Grained Encoder-Decoder} that dynamically fuses the knowledge embedding of entities and attributes in  entity-attribute KG with  token sequence to obtain KG-informed token representation. At last, a \textbf{Constrained Decoding} module and a \textbf{Entity State Changes Classifier Reward}  module are used to improve the correlation and coherence of output.

\subsection{Entity-Attribute Retrieval and Scorer}
% \lifu{Using knowledge acquisition as the title of a subsection is not meaningful enough. People won't be able to get the main idea of this subsection directly from such titles}

% \lifu{the following sentence is meaningless}
% In this section, we explain how to construct the entity-attribute KG.

% \lifu{discuss motivation or goal first, then what you do}
In this section, we explain how to create the entity-attribute KG by utilizing the entities and attributes related to sentences description from the large commonsense KG in two steps: retrieving and scoring.

\paragraph{Retrieving}
We first retrieve the candidate entities and attributes that are in the center of the description anchors from the KG.
%%%%
To better acquire richer entity/attributes knowledge, we leverage ConceptNet~\cite{speer2017conceptnet}, a general KG covering  abundant knowledge with 471,6604 English entities. Specifically, given the action description $x$\footnote{We obtain the candidate entities based on the context and query.
Reason: It is easy to get the relevant entities by the anchor entity in the historical description (context), such as in Figure.\ref{fig:whole framework}, the model just needs  two hops to get the relevant entities by the entity \textit{person}, while the model needs 3 hops to get the entities in the center of \textit{you}. On the other hand, this way can help the model provide richer knowledge information.},
% \lifu{confirm, and did you also extract anchor words from the context and why?} 
we find all the spans in $x$ that are included as entities in ConceptNet, and take each span as an anchor to retrieve the connected entities within $H$ hops in ConceptNet. The candidate entity set is denoted as $E_{x}$.  the $E_{x}$ with their relations naturally forms a \textsl{retrieved KG}.
%%%%%%%
\paragraph{Scoring}
In Retrieving, there are hundreds or thousands of neighboring nodes are retrieved, which provides us not only rich information but also less relevant entities that may be misleading the generation progress. For instance, in the entity-attribute KG of Figure \ref{fig:whole framework}, the retrieved  entities \textit{rich} and \textit{coach} are not relevant to the input description or excepted output. Based on this fact, we train two  BERT-based ranking models $f(.)$ ~\cite{li2022sskgqa} as the scorers (\textsl{entity scorer} and \textsl{attribute scorer}) to semantically obtain the  entity knowledge and attribute knowledge  that are most relevant to the action description.
%%%%%%%%%%%%
For each scorer, it takes the action description $x$ and $E_{x}$ as input, and outputs a score $f(x,e_i)$ indicating whether candidate entity $e_i \in E_{x}$ is related to $x$.
 
To optimize the scorers,  we construct an entity selection training set that consists of $\langle x,ge^p\rangle$ ($ge^p$ is the ground entity set of $x$),  and an attribute selection training set that consists of $\langle x,ga^p\rangle$ ($ga^p$ is the ground attribute set of $x$). More specifically, for the entity scorer, we take the $ge^p$ to construct the positive sample and randomly  select the entities $ge^n$ from $E_{x}-ge^p$, and then use the triplet loss to reduce the distance between $f(x)$ and $f(ge^p_j)$, while enlarging the distance between $f(x)$ and $f(ge^n_j)$.  We utilize the same way to create the attribute scorer. 
%%%%%%%%%%%%
Next, we apply these two scorers to obtain the entity set $SE_x$ and attribute set $SA_x$ that are most relevant to $x$. Finally, the entity-attribute KG is constructed by removing the noise whose score is less than a threshold in the retrieved KG \footnote{In the building progress of entity-attribute KG, we remove the single nodes.}.
As suggested  in \newcite{liu2021kg},  we discuss the model performance with two different score values as shown in Section \ref{con:Impact of Knowledge}.  For more detail about these two scorers and entity-attribute KG, please refer to the section Appendix.\ref{Filter-building}.

 % Given a particular action description, such as the input description in Figure~\ref{fig:whole framework},
 % we aim to first retrieve a candidate set of entities and attributes that are potentially related to the state changes caused by the action. 
 
 % \lifu{this is not a motivation. Motivation should be the intuition of why the entities with state changes are 1-hop or 2-hop related to the anchor entities, and then why we use conceptnet to retrieve the 1-hop/2-hop related entities/attributes}

 % \lifu{we need to provide a detailed description of the motivation of retrieving 1-hop/2-hop entities from ConceptNet. Why the relevant entities/attributes are within 1-hop / 2-hop of the anchor entities? why this approach can help retrieve the entities/attributes that are related to state changes?}

% \lifu{motivation why we design filters instead of using them all}

%\lifu{edited until here}

\subsection{Dynamic Knowledge Grained Encoder-Decoder Modeling (DKGED)}
% \lifu{KnowledgeTransformer is also not meaningful or accurate enough. It cannot indicate the core idea and can have many different interpretations.}
% \lifu{here since incorporating knowledge to the seq-to-seq model is complicated, you can provide an overview of the whole framework, then discuss each component in detail, e.g., graph encoder to encode the knowledge, integrating knowledge in decoder, etc.}
% Intuitively, when asked to write the entity and attribute of an action description, humans will always  call to mind the relevant entity and attribute set about this action separately. In this paper, we propose DKGED to simulate this behavior.
We propose a DKGED to efficiently extract the knowledge-informed feather, and predict the token step by step.
%%%%%%%%%%%%
Given input $\langle x,SE_x,SA_x,\mathbf{s}\rangle$, the DKGED learns a set of parameters $\theta$ by maximizing the likelihood $P(\mathbf{s}|x;\theta)$, which is calculated as the product of the conditional probability of all target tokens in different decoding position:
\begin{align}
% \nonumber\\
P(\mathbf{s}|x;\theta)=\prod_{i=1}^{len(\mathbf{s})}
\left\{ \begin{aligned} 
P(\mathbf{s}|\mathbf{s}_{<i},(x,SE_x);\theta) & & i\in\{[e_k^b,e_k^e]\}\\ 
P(\mathbf{s}|\mathbf{s}_{<i},(x,SA_x);\theta) & & i\in\{[a_l^b,a_l^e]\}\\
P(\mathbf{s}|\mathbf{s}_{<i},x)& & others\\
\end{aligned} \right.
\end{align}
where $\mathbf{s}_i$ represent the $i$-th token of sequence $\mathbf{s}$, 
$\mathbf{s}_{<i}$ represents all the tokens before the $i$-th token.
$e^b$/$e^e$ is the start/end token position \footnote{In the generating progress, these positions can be made by the position of the symbols in the template, such as the position of \textit{of, was}.} of the $k$-th entity $e_k$, $a^b$/$a^e$ is the start/end token position of the $l$-th attribute $a_l$, 
%%%%%%%%%%
% The difference between the standard Transformer and DKGED is the cross-attention calculation, as shown in Figure.\ref{fig:whole framework}.
% The most important characteristic of the DKGED is that it can  dynamically model the entity-attribute information and action description when generating the element at a different position. This operation is achieved by our proposed Dynamic Knowledge Aggregator (DKA).
%%%%%%%%%%%%
%  So in this section, we will give an overview  of our proposed DKGED model and the DKA will be introduced in the next section.
%  %%
% As shown in Figure.\ref{fig:whole framework},
% our proposed encoder-decoder model is designed as a multi-layer transformer-based model which 
% DKGED accepts a token description $x$, the entity set $SE_x$ and attribute set $SA_x$ as input. The output of DKGED is a probability distribution over  the different token positions. It is calculated by:
%%%%%%%%%%
% \textbf{s_{<j}},(x,SE_A)
% More specially, the $x, SA_x,SE_x$ is firstly encoded by a traditional Transformer-based text encoder. 
% Next,the relational Graph Convolutional Network (RGCN) \cite{schlichtkrull2018modeling} is regarded as the graph convolution to encode the interaction information of entities and attributes. By the RGCN, the $SE_x$ and $SA_x$ will be encoded as $\bm{SE_x} \in \mathbb{R}^{z \times d}$ and $\bm{SA_x} \in \mathbb{R}^{t \times d}$ separately, where $z$ is the length of $\bm{SE_x}$, $t$ is the length of $\bm{SA_x}$, $d$ is the embedding dimension.
% The output of the text encoder $\bm{H_x}$ is further used as input for a decoder module \textsl{Dynamic Knowledge Aggregator} that dynamically combines the  $\bm{SE_x}$, $\bm{SA_x}$, $\bm{H_x}$ and previous information about $\mathbf{s}_{<i}$ to predict the token at position $i$.   
% Our proposed Encoder-Decoder model uses the same text encoder as the baseline T5 model. The significant difference lies in the decoder,
% so in the next section, we will describe the decoder module \textsl{dynamic knowledge aggregator} in detail.
where, the $x, SE_x,SA_x$ is firstly encoded by the following function:
\begin{align}
&\mathbf{X}=T5Encoder(x) \nonumber\\
&\mathbf{SE_x},\mathbf{SA_x}=RGCN(SE_x,SA_x)
\end{align}
To provide the interaction information for the entities and attributes, in this work, we choose the relational Graph Convolutional Network $RGCN$ which is provided to be effective in \cite{ribeiro2021structural}.
%%%%%%%%%%%%%
The $\mathbf{X}$ is further used as input for a decoder module \textsl{Dynamic Knowledge Aggregator} that dynamically combines the  $\mathbf{SE_x}$, $\bm{SA_x}$, $\mathbf{X}$ and information about $\mathbf{s}_{<i}$ to predict the token at position $i$. Our proposed Encoder-Decoder model uses the same text encoder as the baseline T5 model. The significant difference lies in the decoder, so in the next section, we will describe the decoder module \textsl{dynamic knowledge aggregator} in detail.

\subsubsection{Dynamic Knowledge Aggregator (DKA)}
% \lifu{again, don't use too many such names. Awkward and not meaningful}
% Our Dynamic Knowledge Aggregator (DKA) aims to efficiently leverage  the different knowledge when decoding different tokens.
The most important characteristic of the DKA is that it can  dynamically model the entity-attribute information and action description when generating the element at a different position.
% Recall, the output of the $l$-th standard attention network is defined as:
% \begin{align}
% &\mathbf{Q}_l=\mathbf{H}_{l-1}^q \mathbf{W}_l^{q}, \mathbf{K}_l=\mathbf{H}_{l-1}^{kv}\mathbf{W}_l^{k}, \mathbf{V}_l=\mathbf{H}_{l-1}^{kv}\mathbf{W}_l^{v} \nonumber\\
% &\overline{\mathbf{H}}^{l}=\mu(\frac{\mathbf{Q}_{l}\mathbf{K}_{l}^\textup{T}}{\sqrt{d_k}} )\mathbf{V}_{l}
% 	\label{A_h}
% \end{align}
% \noindent where $\mathbf{W}_l^q, \mathbf{W}_l^k, \mathbf{W}_l^v\in \mathbb{R}^{d_{model} \times d_k}$ denote the learnable weight matrices, $\mu$ denotes the $softmax$ function. $d_{model}$ is the model dimension, $d_k$ is the head dimension. 
% $H^q$ and $H^{kv}$ are two input vectors for attention, with $H^{kv}$ serving as key and value, $H^q$  serving as query.
% As our dynamic knowledge aggregator try to generate the tokens by using different knowledge, specifically, the aggregator  uses the entity knowledge with description  knowledge to generate the entity and uses the attribute knowledge with description  knowledge to generate the attribute.
% First, we define the key-value pair and query for different knowledge as follows,
% \begin{align}
% &Q_l^t=SN(Y^{l-1}) W_l^{t} \nonumber\\
% &K_l^q=\bm{H_x}^{l-1}W_l^{k^q}, V_l^q=\bm{H_x}^{l-1}W_l^{v^q} \nonumber\\
% %%%%%%%%%%%%%
% &K_l^e=\bm{SE_x}^{l-1}W_l^{k^e}, V_l^e=\bm{SE_x}^{l-1}W_l^{v^e}\nonumber\\
% %%%%%%%%%%
% &K_l^a=\bm{SA_x}^{l-1}W_l^{k^a}, V_l^a=\bm{SA_x}^{l-1}W_l^{v^a}
% \end{align}
% \noindent where $(W_l^q, W_l^k, W_l^v)\in \mathbb{R}^{d_{model} \times d_k}$ are learnable weight matrices for different input knowledge. 
% $SN$ denotes the combined operation of
% self-attention with the norm Layer. $Y$ is the target state change.
% So, when generating the token belonging to the attribute at step $i$,
% the output of a cross-attention head ${A}_h^i$ in layer $l$ is calculated as:


% \begin{align}
% &(\tilde{A}_h^q)_l^i=\mu\left(\frac{(Q_{t}^q)^i (K_{l}^q) ^\textup{T}}{\sqrt{d_k}} \right)V_{l}^q \nonumber\\
% &(\tilde{A}_h^a)_l^i=\mu\left(\frac{(Q_{t}^q)^i (K_{l}^a) ^\textup{T}}{\sqrt{d_k}} \right)V_{l}^a\nonumber\\
%  &(\tilde{A}_h^i)_l=(\tilde{A}_h^q)_l^i+(\tilde{A}_h^a)_l^i
% \end{align}

%  when generating the token belonging to entity  at step $i$,
% the output of a cross-attention head $\tilde{A}_h^i$ is calculated as:
% %adaptive weighted attention matrix is calculated as follow.
% \begin{align}
% &(\tilde{A}_h^q)_l^i=\mu\left(\frac{(Q_{t}^q)^i (K_{l}^q) ^\textup{T}}{\sqrt{d_k}} \right)V_{l}^q\nonumber\\ 
% &(\tilde{A}_h^e)_l^i=\mu\left(\frac{(Q_{t}^q)^i (K_{l}^e) ^\textup{T}}{\sqrt{d_k}} \right)V_{l}^e\nonumber\\
% &(\tilde{A}_h^i)_l=(\tilde{A}_h^q)_l^i+(\tilde{A}_h^e)_l^i
%  \end{align}
% % where
% % $(\tilde{A}_h^e)^i$ is calculated by the CA3-E in  Figure  \ref{fig:MKDDecoder}.
% For the other tokens, the $\tilde{A}_h^i$ is calculated just by the question information $(\tilde{A}_h^q)^i$.

The DKA consists of $L$ identical layers. The output  of the $l$-th layer can be formalized as follows:
\begin{align} 
&\mathbf{\bar{H}}_i^l=LN(MultiATTN(CM(\mathbf{H}_i))+\mathbf{H}_i^{l-1})\nonumber\\
&\mathbf{\breve{H}}_i^l=LN(CrossATTN(\mathbf{\bar{H}}_i^l,\mathbf{X}+\mathbf{SA}_x)+\mathbf{\bar{H}}_i^l)\nonumber\\
&\mathbf{\dot{H}}_i^l=LN(CrossATTN(\mathbf{\bar{H}}_i^l,\mathbf{X}+\mathbf{SE}_x)+\mathbf{\bar{H}}_i^l)\nonumber\\
&\mathbf{\ddot{H}}_i^l=LN(CrossATTN(\mathbf{\bar{H}}_i^l,\mathbf{X})+\mathbf{\bar{H}}_i^l)\nonumber\\
&\mathbf{{H}}_i^l=
\left\{ \begin{aligned} 
LN(FFN(\mathbf{\breve{H}}_i^l)+\mathbf{\breve{H}}_i^l) & & i\in\{[e_k^b,e_k^e]\}\\ 
LN(FFN(\mathbf{\dot{H}}_i^l)+\mathbf{\dot{H}}_i^l) & & i\in\{[a_l^b,a_l^e]\}\\
LN(FFN(\mathbf{\ddot{H}}_i^l)+\mathbf{\ddot{H}}_i^l)& & others\\
\end{aligned} \right.  \nonumber\\
&\mathbf{{H}}^l=[\mathbf{{H}}_0^l,\mathbf{{H}}_1^l,...,\mathbf{{H}}_i^l] 
\label{main function}
\end{align}
where $\mathbf{H^0}=EMB(\mathbf{s})$ denotes the initial representation from the embedding layer about the target $\mathbf{s}$. $CM$ represents the causal mask mechanism that is used in the standard Transformer. the implementation of cross attention $CrossAttentioin$ is the same as the traditional multi-head attention $MultiATTN$. $LN$ and $FFN$ denote the  Layer Normalization  and Feed Forward Layer  separately. As shown in equation \ref{main function} and the right chart of Figure.\ref{fig:whole framework}, 
DKA could use the question knowledge $\mathbf{\breve{H}}_i^l$, entity knowledge $\mathbf{\ddot{H}}_i^l$ and attribute $\mathbf{\dot{H}}_i^l$ to decoder the entity, attribute at different position $i$ separately.
The output target sequence is generated on the output hidden state $\mathbf{{H}}^L$ from the top layer of the decoder:
\begin{align} 
&P(\mathbf{Y}|((\mathbf{X},\mathbf{SE}_x,\mathbf{SA_x});\theta)=softmax(\mathbf{W}\mathbf{{H}}^L)
\label{main function}
\end{align}
where $\mathbf{W}$ is the project weight parameter, which maps the hidden state to the probability in the vocabulary space.

\subsection{Constrained Decoding}
Given the hidden sequence, the encoder-decoder model needs to generate the linearized entity state changes token by token. One straightforward idea is to use greedy decoding to choose the token with the highest predicted score $p(\mathbf{s}_i|\mathbf{s}_{<i},x)$ at decoding step $i$. In each step $i$, the candidate token is the whole token set $V$ of the language model. Unfortunately, we find some candidate tokens mislead the token selection of the model that are irrelevant to the action description, and further cause the model to generate the state changes that are irrelevant to the description. 
%%%%%%%%%%%%%%

So the motivation of our Constrained Decoding is to filter the noise in the candidate token set when generating the token step by step.
Specifically, (1) 
We remove the tokens whose surface name contains the special symbol, such as  \textit{cărți, \$9} in the candidate token set. (2)
a relevant score $\gamma$  is further calculated between each token $c \in V$  and  the action description $x$. At last, we remove the token whose relevant score is less than a threshold: 
\begin{align} 
\gamma (c,x)=\max_{}(\mathbf{c},\{\mathbf{w_0},\mathbf{w_1},...,\mathbf{w_j}\}), w_j \in x \label{score}
\end{align}
where $w_i$ is the word in $x$, $j$ is the words length of $x$,  $\mathbf{c}$ and $\mathbf{w_i}$ is the  embedding of  $c$ and $w_i$,  the embedding is calculated by the pre-trained T5 model. $\gamma$ is the cosine similarity function.  Please refer to section Appendix\ref{Constrained Decoding} for more detail.



\subsection{Entity State Changes Classifier Reward}
% Qualitative evaluation showed some of the state changes generated were not reasonable, making them unsuitable for the task of generating the tuples easily. For example, In generated state changes: \textit{texture of activity was optional before and organized afterwards}, the \textit{texture} is not the attribute of \textit{activity}.
 Qualitative evaluation showed some of the state changes generated  were not reasonable. For example, generated \textit{ composition of flowers were in dead flowers before and fresh flowers afterwards}, the state changes \textit{dead/fresh flowers} are not relevant to the attribute \textit{composition}.

To address this problem, same as \cite{lai2021thank}, we use a \textsl{classification confidence reward} to encourage the model to generate the  relevant entity state changes in the confidence of a \textsl{entity state changes classifier (ESCC)}.
Basically, the state change would be fed as input to the classifier, and the output of the classifier is predicted as "1" (state change is logical) or "0" (state change is not logical). The whole network is fully differentiable and can be optimized by minimizing the traditional cross-entropy. For the detail about the ESCC, please refer to section Appendix.\ref{tuple classifcation}.



The confidence of classifier $TC$ is formulated as:
\begin{align} 
p(l_i|y)=softmax_i(T5Encoder(y,\theta))
\end{align}
where, $l_i$ is $0$ or $1$, and refers relevant ESC or irrelevant ESC  respectively.  $\theta$ are the parameters of $ESCC$. The reward is computed by:
\begin{align} 
R_{cls}= p_s(p(l_1|y)-p(l_0|y))
\end{align}
where $y$ is the generated target state changes sampled from the model's candidate token set at each step in decoding. $p_s$ is the probability of sampled tokens.
%%%%%%%%
And then the reward is used for policy learning, the policy gradient is calculated by:
\begin{align} 
\nabla_{\phi}J(\phi)=E[R_{cls} \cdot\nabla_{\phi}log(P(y|x;\phi)) ]
\end{align}
Where $\phi$ represents the model parameters.
Hence, the overall loss function for our proposed knowledge model is:

\begin{align}
&L_{CE}=-\sum_{i=1}^{k}log(P(y_i|y_{<i},x))  \nonumber\\ 
&L_{RL}=-\frac{1}{t}\sum_{i=1}^{t}R_{cls}^{i}\nonumber\\ 
&L=(1-\lambda)\cdot L_{CE} +\lambda \cdot L_{RL}
\label{eq:reward}
\end{align}


where $L_{CE}$ is the cross-entropy loss used to optimize the network in addition to rewards.  where $\lambda\in[0,1]$ is a tunable parameter, it will be discussed in our experiments.

==> results_2022_10_26.tex <==


\section{Experiments}

\begin{table*}[ht]
	\centering
		
	\renewcommand\arraystretch{1.3}
	\scalebox{0.9}
 {
	\begin{tabular} {c|c|ccc|ccc|ccc}
		\hline 
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ExactMatric}& \multicolumn{3}{c}  {BLEUMetric}& \multicolumn{3}{c}  {ROUGEMetric}  \\
		\hline
		 model&max-Length& Prec &  recall &F1&  Prec &  recall &F1 &  Prec &  recall &F1  \\ 
		\hline	
		Paper gpt2 base&none & & & 3.6& & &13.4 & &&28.2\\
		GitHub-gpt2-base&400&8.82 & 7.00&4.13 &22.85 &19.08 & 16.38& 39.54&35.18 &32.66\\
        my-gpt2-base&400&8.85& 6.76&3.87 &22.77 &18.64 & 15.97& 39.75&34.51 &32.29\\
          t5-large-baseline&400& \textbf{15.22 } & \textbf{7.46}  &  \textbf{5.64} & \textbf{31.30} &\textbf{20.33} & \textbf{19.29}& \textbf{47.83}&\textbf{35.97} &\textbf{35.52}\\
       
          % t5-large-baseline-&400& 13.16   &7.46    & 5.06   & 32.02  &  22.42& 21.09 & 48.49 & 38.22 & 37.44\\
		
       
        % method1-add-attr&400& 16.85   &7.57   &6.30    &34.49   &22.06  & 21.53 &50.4 &36.88 & 36.99\\
        % method2-attr&400& 25.11   &6.15  &5.53    &39.54   &18.60 & 18.13 &54.37 &32.57 & 32.74\\
        \hline
        score$>$0.5&&    &   &    &   &  &  & & & \\
        
        %  train(q,e)-pre(q,e)&400& 17.49   & 7.86  &6.19    &34.95   &21.94  &21.00  &50.66 & 36.58& 36.41\\
        % train(q,a)-pre(q,a)&400& low-explode   &   &    &   &  &  & & & \\

        % train(q,a,e)-pre(q,a)&400& 26.34  & 6.83 & 5.70   & 42.34  & 19.44 &19.19  & 56.10&33.05 &33.07 \\
        
        %  train(q,a,e)-pre(q,e)&400& 20.48  & 7.96 & 7.01   & 37.79  & 22.07 &21.92  & 53.19&36.78 &37.17 \\
        %  train(q,a,e)-pre(q,a,e)&400& 23.22  & 7.03 & 5.64   & 39.36  & 20.58 &19.70  & 53.83&34.37 &34.00 \\
        %  train(q,a,e)-pre(q)&400&\textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\


         
        
         train(q,a,e)-pre(q,a)&400& 26.10  & 7.28 & 6.42   & 42.11  & 20.19 &20.20  & 56.94&34.35 &34.84 \\
          train(q,a,e),pre(q?)&400&\textbf{ 19.77} &\textbf{ 7.67} & \textbf{6.92}  &\textbf{37.66}  &\textbf{22.05} &\textbf{22.17}  &\textbf{53.12} &\textbf{36.63} &\textbf{37.37} \\
         train(q,a,e)-pre(q,a2-0.01)&400& 18.75  & 7.30 & 6.52   & 36.59  & 21.77 &21.77 & 52.60&36.73 &37.46 \\
         
         train(q,a,e)-pre(q,e)&400& 20.91  & 7.55 & 6.64   & 38.03  & 21.67 &21.53  & 53.20&36.12 &36.49 \\
         train(q,a,e)-pre(q,a,e)-all2&400& \textbf{19.82}  &\textbf{ 7.56} & \textbf{6.82 }  & \textbf{37.65}  & \textbf{21.94} &\textbf{22.05} & \textbf{53.17}&\textbf{36.59} &\textbf{37.28}\\
        \hline
        introduce e,a is the best&&    &   &    &   &  &  & & & \\
            train(q,e)-pre(q,e)&400& 17.49   & 7.86  &6.19    &34.95   &21.94  &21.00  &50.66 & 36.58& 36.41\\
        train(q,a)-pre(q,a)&400&   &   &    &   &  &  & & & \\
         train(q,a,e)-pre(q,a,e)-all2&400& \textbf{19.82}  &\textbf{ 7.56} & \textbf{6.82 }  & \textbf{37.65}  & \textbf{21.94} &\textbf{22.05} & \textbf{53.17}&\textbf{36.59} &\textbf{37.28}\\
         

       \hline
	\end{tabular}
 }
	\caption{Model performance}
\label{con:model-performance}
\end{table*}

